Impostor Networks for Fast Fine-Grained Recognition

In this work we introduce impostor networks, an architecture that allows to perform fine-grained recognition with high accuracy and using a light-weight convolutional network, making it particularly suitable for fine-grained applications on low-power and non-GPU enabled platforms. Impostor networks compensate for the lightness of its `backend' network by combining it with a lightweight non-parametric classifier. The combination of a convolutional network and such non-parametric classifier is trained in an end-to-end fashion. Similarly to convolutional neural networks, impostor networks can fit large-scale training datasets very well, while also being able to generalize to new data points. At the same time, the bulk of computations within impostor networks happen through nearest neighbor search in high-dimensions. Such search can be performed efficiently on a variety of architectures including standard CPUs, where deep convolutional networks are inefficient. In a series of experiments with three fine-grained datasets, we show that impostor networks are able to boost the classification accuracy of a moderate-sized convolutional network considerably at a very small computational cost.

==> plots/timings.tex <==
% This file was created by matplotlib2tikz v0.6.15.
\begin{tikzpicture}[scale=0.7]

\definecolor{color1}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color0}{rgb}{1,0.498039215686275,0.0549019607843137}

\begin{groupplot}[group style={group size=2 by 2}]
\nextgroupplot[
title={cpu timings},
ylabel={time, [ms]},
xmin=-0.59, xmax=3.59,
ymin=0, ymax=363.443398476039,
xtick={0,1,2,3},
xticklabels={squeezenet,alexnet,resnet18,resnet50},
tick align=outside,
tick pos=left,
x grid style={lightgray!92.026143790849673!black},
y grid style={lightgray!92.026143790849673!black},
%legend entries={{knn},{cnn}},
legend cell align={left},
legend style={at={(0.03,0.97)}, anchor=north west, draw=white!80.0!black}
]
\draw[fill=color0,draw opacity=0] (axis cs:-0.4,0) rectangle (axis cs:0.4,84.00690555575);
\draw[fill=color0,draw opacity=0] (axis cs:0.6,0) rectangle (axis cs:1.4,61.03396415713);
\draw[fill=color0,draw opacity=0] (axis cs:1.6,0) rectangle (axis cs:2.4,162.80949115707);
\draw[fill=color0,draw opacity=0] (axis cs:2.6,0) rectangle (axis cs:3.4,346.13656997718);
\draw[fill=color1,draw opacity=0] (axis cs:-0.4,0) rectangle (axis cs:0.4,79.2330503464);
\draw[fill=color1,draw opacity=0] (axis cs:0.6,0) rectangle (axis cs:1.4,56.0464859009);
\draw[fill=color1,draw opacity=0] (axis cs:1.6,0) rectangle (axis cs:2.4,158.102035522);
\draw[fill=color1,draw opacity=0] (axis cs:2.6,0) rectangle (axis cs:3.4,341.590046883);
\nextgroupplot[
title={gpu timings},
xmin=-0.59, xmax=3.59,
ymin=0, ymax=22.3839819431645,
xtick={0,1,2,3},
xticklabels={squeezenet,alexnet,resnet18,resnet50},
tick align=outside,
tick pos=left,
x grid style={lightgray!92.026143790849673!black},
y grid style={lightgray!92.026143790849673!black}
]
\draw[fill=color0,draw opacity=0] (axis cs:-0.4,0) rectangle (axis cs:0.4,5.146503448488);
\draw[fill=color0,draw opacity=0] (axis cs:0.6,0) rectangle (axis cs:1.4,4.560470581052);
\draw[fill=color0,draw opacity=0] (axis cs:1.6,0) rectangle (axis cs:2.4,9.379506111146);
\draw[fill=color0,draw opacity=0] (axis cs:2.6,0) rectangle (axis cs:3.4,21.318078041109);
\draw[fill=color1,draw opacity=0] (axis cs:-0.4,0) rectangle (axis cs:0.4,4.55951690674);
\draw[fill=color1,draw opacity=0] (axis cs:0.6,0) rectangle (axis cs:1.4,3.97443771362);
\draw[fill=color1,draw opacity=0] (axis cs:1.6,0) rectangle (axis cs:2.4,8.79204273224);
\draw[fill=color1,draw opacity=0] (axis cs:2.6,0) rectangle (axis cs:3.4,20.7340717316);
\nextgroupplot[
xlabel={accuracy, [\%]},
ylabel={time, [ms]},
xmin=64.2937067631287, xmax=87.7919708775234,
ymin=41.4903836707271, ymax=18148.7055203752,
ymode=log,
tick align=outside,
tick pos=left,
x grid style={lightgray!92.026143790849673!black},
y grid style={lightgray!92.026143790849673!black},
%legend entries={{cnn},{loose},{baseline}},
legend cell align={left},
legend style={at={(0.03,0.97)}, anchor=north west, draw=white!80.0!black}
]
\addplot [only marks, draw=color1, fill=color1, colormap/viridis]
table{%
x                      y
+7.072000000000000e+01 +7.923305034640001e+01
+6.558000000000000e+01 +5.604648590090000e+01
+7.961000000000000e+01 +1.581020355220000e+02
+8.234999999999999e+01 +3.415900468830000e+02
};
\addplot [only marks, draw=color0, fill=color0, colormap/viridis]
table{%
x                      y
+7.601000000000001e+01 +8.400690555575001e+01
+6.730000000000000e+01 +6.103396415713000e+01
+8.058000000000000e+01 +1.628094911570700e+02
+8.214000000000000e+01 +3.461365699771800e+02
};
\addplot [only marks, draw=black, fill=black, colormap/viridis]
table{%
x                      y
+8.500000000000000e+01 +3.643340000000000e+03
+8.540000000000001e+01 +1.342641000000000e+04
+8.540000000000001e+01 +5.406380000000000e+03
+8.650000000000000e+01 +7.169420000000000e+03
+8.540000000000001e+01 +6.610030000000001e+03
+8.650000000000000e+01 +8.744590000000000e+03
};
\addplot [semithick, color0, forget plot]
table {%
70.72 79.2330503464
76.01 84.00690555575
};
\addplot [semithick, color0, forget plot]
table {%
65.58 56.0464859009
67.3 61.03396415713
};
\addplot [semithick, color0, forget plot]
table {%
79.61 158.102035522
80.58 162.80949115707
};
\addplot [semithick, color0, forget plot]
table {%
82.35 341.590046883
82.14 346.13656997718
};
\draw[] (axis cs:70.72,79.2330503464) -- (axis cs:70.72,79.2330503464);
\node at (axis cs:70.72,79.2330503464)[
  scale=0.5,
  anchor=base,
  text=black,
  rotate=0.0
]{ squeezenet};
\draw[] (axis cs:65.58,56.0464859009) -- (axis cs:65.58,56.0464859009);
\node at (axis cs:65.58,56.0464859009)[
  scale=0.5,
  anchor=base,
  text=black,
  rotate=0.0
]{ alexnet};
\draw[] (axis cs:79.61,158.102035522) -- (axis cs:79.61,158.102035522);
\node at (axis cs:79.61,158.102035522)[
  scale=0.5,
  anchor=base,
  text=black,
  rotate=0.0
]{ resnet18};
\draw[] (axis cs:82.35,341.590046883) -- (axis cs:82.35,341.590046883);
\node at (axis cs:82.35,341.590046883)[
  scale=0.5,
  anchor=base,
  text=black,
  rotate=0.0
]{ resnet50};
\draw[] (axis cs:85,3643.34) -- (axis cs:85,3643.34);
\node at (axis cs:85,3643.34)[
  scale=0.5,
  anchor=north west,
  text=black,
  rotate=0.0
]{ 1};
\draw[] (axis cs:85.4,13426.41) -- (axis cs:85.4,13426.41);
\node at (axis cs:85.4,13426.41)[
  scale=0.5,
  anchor=north west,
  text=black,
  rotate=0.0
]{ 2};
\draw[] (axis cs:85.4,5406.38) -- (axis cs:85.4,5406.38);
\node at (axis cs:85.4,5406.38)[
  scale=0.5,
  anchor=north west,
  text=black,
  rotate=0.0
]{ 3};
\draw[] (axis cs:86.5,7169.42) -- (axis cs:86.5,7169.42);
\node at (axis cs:86.5,7169.42)[
  scale=0.5,
  anchor=north west,
  text=black,
  rotate=0.0
]{ 4};
\draw[] (axis cs:85.4,6610.03) -- (axis cs:85.4,6610.03);
\node at (axis cs:85.4,6610.03)[
  scale=0.5,
  anchor=north west,
  text=black,
  rotate=0.0
]{ 5};
\draw[] (axis cs:86.5,8744.59) -- (axis cs:86.5,8744.59);
\node at (axis cs:86.5,8744.59)[
  scale=0.5,
  anchor=north west,
  text=black,
  rotate=0.0
]{ 6};
\nextgroupplot[
xlabel={accuracy[\%]},
xmin=64.2937067631287, xmax=87.7919708775234,
ymin=3.09994624690207, ymax=448.017564850894,
ymode=log,
tick align=outside,
tick pos=left,
x grid style={lightgray!92.026143790849673!black},
y grid style={lightgray!92.026143790849673!black}
]
\addplot [only marks, draw=color1, fill=color1, colormap/viridis]
table{%
x                      y
+7.072000000000000e+01 +4.559516906740000e+00
+6.558000000000000e+01 +3.974437713620000e+00
+7.961000000000000e+01 +8.792042732240001e+00
+8.234999999999999e+01 +2.073407173160000e+01
};
\addplot [only marks, draw=color0, fill=color0, colormap/viridis]
table{%
x                      y
+7.601000000000001e+01 +5.146503448488000e+00
+6.730000000000000e+01 +4.560470581052000e+00
+8.058000000000000e+01 +9.379506111146000e+00
+8.214000000000000e+01 +2.131807804110900e+01
};
\addplot [only marks, draw=black, fill=black, colormap/viridis]
table{%
x                      y
+8.500000000000000e+01 +9.331000000000000e+01
+8.540000000000001e+01 +3.492300000000000e+02
+8.540000000000001e+01 +1.457500000000000e+02
+8.650000000000000e+01 +1.981900000000000e+02
+8.540000000000001e+01 +1.821300000000000e+02
+8.650000000000000e+01 +2.478500000000000e+02
};
\addplot [semithick, color0, forget plot]
table {%
70.72 4.55951690674
76.01 5.146503448488
};
\addplot [semithick, color0, forget plot]
table {%
65.58 3.97443771362
67.3 4.560470581052
};
\addplot [semithick, color0, forget plot]
table {%
79.61 8.79204273224
80.58 9.379506111146
};
\addplot [semithick, color0, forget plot]
table {%
82.35 20.7340717316
82.14 21.318078041109
};
\draw[] (axis cs:70.72,4.55951690674) -- (axis cs:70.72,4.55951690674);
\node at (axis cs:70.72,4.55951690674)[
  scale=0.5,
  anchor=base west,
  text=black,
  rotate=0.0
]{ squeezenet};
\draw[] (axis cs:65.58,3.97443771362) -- (axis cs:65.58,3.97443771362);
\node at (axis cs:65.58,3.97443771362)[
  scale=0.5,
  anchor=base west,
  text=black,
  rotate=0.0
]{ alexnet};
\draw[] (axis cs:79.61,8.79204273224) -- (axis cs:79.61,8.79204273224);
\node at (axis cs:79.61,8.79204273224)[
  scale=0.5,
  anchor=base west,
  text=black,
  rotate=0.0
]{ resnet18};
\draw[] (axis cs:82.35,20.7340717316) -- (axis cs:82.35,20.7340717316);
\node at (axis cs:82.35,20.7340717316)[
  scale=0.5,
  anchor=base west,
  text=black,
  rotate=0.0
]{ resnet50};
\draw[] (axis cs:85,93.31) -- (axis cs:85,93.31);
\node at (axis cs:85,93.31)[
  scale=0.5,
  anchor=north west,
  text=black,
  rotate=0.0
]{ 1};
\draw[] (axis cs:85.4,349.23) -- (axis cs:85.4,349.23);
\node at (axis cs:85.4,349.23)[
  scale=0.5,
  anchor=north west,
  text=black,
  rotate=0.0
]{ 2};
\draw[] (axis cs:85.4,145.75) -- (axis cs:85.4,145.75);
\node at (axis cs:85.4,145.75)[
  scale=0.5,
  anchor=north west,
  text=black,
  rotate=0.0
]{ 3};
\draw[] (axis cs:86.5,198.19) -- (axis cs:86.5,198.19);
\node at (axis cs:86.5,198.19)[
  scale=0.5,
  anchor=north west,
  text=black,
  rotate=0.0
]{ 4};
\draw[] (axis cs:85.4,182.13) -- (axis cs:85.4,182.13);
\node at (axis cs:85.4,182.13)[
  scale=0.5,
  anchor=north west,
  text=black,
  rotate=0.0
]{ 5};
\draw[] (axis cs:86.5,247.85) -- (axis cs:86.5,247.85);
\node at (axis cs:86.5,247.85)[
  scale=0.5,
  anchor=north west,
  text=black,
  rotate=0.0
]{ 6};
\end{groupplot}

\end{tikzpicture}
